Query Containment for Highly Expressive Datalog Fragments

The containment problem of Datalog queries is well known to be undecidable. There are, however, several Datalog fragments for which containment is known to be decidable, most notably monadic Datalog and several "regular" query languages on graphs. Monadically Defined Queries (MQs) have been introduced recently as a joint generalization of these query languages. In this paper, we study a wide range of Datalog fragments with decidable query containment and determine exact complexity results for this problem. We generalize MQs to (Frontier-)Guarded Queries (GQs), and show that the containment problem is 3ExpTime-complete in either case, even if we allow arbitrary Datalog in the sub-query. If we focus on graph query languages, i.e., fragments of linear Datalog, then this complexity is reduced to 2ExpSpace. We also consider nested queries, which gain further expressivity by using predicates that are defined by inner queries. We show that nesting leads to an exponentially increasing hierarchy for the complexity of query containment, both in the linear and in the general case. Our results settle open problems for (nested) MQs, and they paint a comprehensive picture of the state of the art in Datalog query containment.

==> lMDL-CRPQ.tex <==
We prove in this paragraph that the problem of containment of
Linear Monadic Datalog over relations or arity less than $2$ in nested-CR2PQs
is in {\sc exspace}.

We will decompose the proof in different parts.
First, we sketch the methods introduced in \cite{}
to proof that the problem of containment of RPQ
in CR2PQ is in {\sc exspace}.
Then, we prove how to extend this result
for the problem of containment of RPQ in nested
CR2PQs. The last step before proving
our main result is to explain how to extend
the containment of Linear Monadic Datalog in CR2PQs.
This results has proved for the first,
Finally, we prove the main result.

\paragraph{Containment of RPQ in CRPQs \cite{}}
Let $x.L.y$ be a RPQ.
Let $Q$ be a CR2PQ. Let $\V$ be the set of variables of $Q$.
In \cite{}, it is proved that if there exists a witness of the not containment of $x.L.y$ in $Q$
then there exists a word satisfying $L$ and not satisfying $Q$.
The main idea of this proof is to rewrite $Q$ in a two way automaton $A_Q$ such that
every word in $L$ accepted by $A_Q$ is accepted by $Q$ and then check the containment of $L$ in $A_Q$.
Without loss of assumptions, we assume that there exists an ordered structure $N$ such that the nodes of a word are $N$, the initial node is $n_0$
and the order of the nodes of a  word are consistent with the order of $N$.
Let $w$ be a word accepted by $Q$. Then there exists a mapping $\nu$ from the variables of $Q$ to the nodes of $w$.
This word and the mapping can be seen as an enriched word, i.e. a word of such that nodes are enriched with sets representing sets of variables of $Q$.
A word is \emph{$Q$-mapped word} iff for each variable  $x$ of $Q$, there exists an unique node with an associated set containing $x$.
In order to build $A_Q$, we first build an automaton $A_{Q,\nu}$ where which recognizes $Q$-mapped words satisfying $Q$.

We now explain the construction of $A_{\nu,Q}$.
Let alphabet $\Sigma'$ equal to $\Sigma \times (2^{\V} \times 2^{\V})$.
Intuitively, a letter $(\alpha, S_1,S_2)$ denotes an edge $(n_i,n_{i+1})$ labeled with
the label $\alpha$ and such that  $S_1$ is mapped exactly the set of variables of $Q$ mapped to $n_i$ by $\nu$ and
$S_2$ is equal to the set of variables of $Q$ mapped to $n_{i+1}$.
Let $x_i.L_i.x_{i+1}$ be a R2PQ which is a conjunct in $Q$.
Let $L'_i$ be the regular language over $\Sigma'$ such that
\begin{itemize}
\item the projection of $L'_i$ over $\Sigma$ is equal to $L_i$
\item the first letters of words accepted by $L'_i$ are of the form $(\alpha,S,S')$ such that $x_i$ is in $P$
\item the last letters of words accepted by $L'_i$ are of the form $(\alpha,S,S'$ such that $x_{i+1}$ is in $P'$.
\end{itemize}
$A_{\nu,x_i.L_i.x_{i+1}}$ is a two way automaton which accepts any word in $\Sigma'^{*}.L'_i.\Sigma'^{*}$.
We can notice that $A_{\nu,x_i.L_i.y_i}$ a two way automaton because $L_i$ use both predicates $\alpha$ and $\alpha^-1$ which authorizes to go
back and forth in the word.
We then construct an automaton $A_{\nu,Q}$ which accepts a word satisfying $Q$ by using $\nu$.
Intuitively, $A_{\nu,Q}$ is the product of the automata $A_{\nu,x_i.L_i.x_{i+1+}}$. We also have to check that the word recognized by $A_{\nu,Q}$
are $Q$-mapped. This can be easily expressed by an automaton $A_{c}$ over $\Sigma'$.
Therefore, $A_{\nu,Q}$ is the product of each $A_{\nu,x_i.L_i.y_i}$ and of $A_c$.
We then do the projection of $A_{\nu,Q}$ over $\Sigma$ to obtain $A_Q$.
A word over the alphabet $\Sigma$ is accepted by $A_Q$ iff there exists a mapping $\nu$ such that the $Q$-mapped word $w_{\nu}$
obtained from $w$ and $\nu$ is recognized by $A_{\nu,Q}$, i.e. that $w,\nu$ satisfies $Q$.

We now prove that $A_Q$ is of size exponential in the input.
First, we can notice that $\Sigma'$ is exponential in the input. However, clearly each automaton $A_{\nu,x_i.L_i.x_{i+1}}$ has a polynomial number
of states as $A_c$. We can translate each of the two way automata $A_{\nu,x_i.L_i.x_{i+1}}$ into equivalent
deterministic finite state automata $A'_{\nu,x_i.L_i.x_{i+1}}$ which has a number of states exponential in the number of $A_{\nu,x_i.L_i.x_{i+1}}$.
It is the same for $A_c$ following result of \cite{}. The product of the $A'_{\nu,x_i.L_i.x_{i+1}}$ and $A_c$ is exponential in the number conjuncts in $Q$.
Therefore, the number of states of $A_{\nu,Q}$ is exponential in the size of the input.
We finish by doing the projection over $\Sigma$. We notice that $A_{\nu,Q}$ is a deterministic finite state automaton.
Therefore, the projection of $A_{\nu,Q}$ over $\Sigma$ is polynomial in the alphabet and the number of states of $A_{\nu,Q}$.
 Thus $A_{Q}$ has a size exponential in the inputs.
Therefore, the containment of $A_L$ and $A_{Q}$ is in {\sc exspace}.
This finishes the proof for the classical case.

\paragraph{Containment of RPQ in nested CR2PQs}
The goal is to reduce this problem to the containment of two automata as in the previous paragraph.
Let $x.L.y$ be RPQ. Let $Q$ be a $k$-nested CR2PQ. Let $C_1 \cdots C_k$ be the subC2RPQs used in $Q$ or in any $C_i$.
Without loss of assumption, we consider that for any subCR2PQ $C_i$, the formula is of the form $x.L.y$ where if $L$ contains a subquery then $L$ is free of starts
or $C_i$ is of the form $x.(C_j)^*.y$ where $C_j$ is a subCR2PQ of $C_i$.
We explain how to build an automaton $A_{C_i}$ by induction on the structure of $C_i$.
We consider the letters $(\alpha,x_{C_i})$, $(\alpha,x_{C_i},y_{C_i})$ and $(\alpha,y_{C_i}$ 
where $\alpha$ is in $\Sigma$. We denote by $\Sigma_{C_i}$, this alphabet. 
For each nested subCR2PQ $C_i$, we now consider the alphabet $\Sigma \cup \Sigma_{C_i} \bigcup_{j \in \sub(i)} \Sigma_{C_{j}}$
as the legitimated alphabet. 















==> linmdatalog-linMQ.tex <==
We prove that the containment of \linmdatalog in \mq is in \ExpSpace.
We reduce our problem to the containment of two nondeterministic automaton of size exponential.
Let $P_1$ and $P_2$ be the two \linmq programs.
Let $\Sigma_{P_1}$ be the alphabet used to encode the word witnesses from $P_1$ as presented by before. 
This alphabet is polynomial in the size of $P_1$. Each letter of this alphabet corresponds to a rule of $P_1$.
We enrich this alphabet to an alphabet $\Sigma_{P_1,P_2}$ containing also the intentional predicates of $P_2$ and the $\lambda$ variables
of $P_2$ explaining which are the intentional predicate assigned to each value.

We want to show that we can run an automaton $A{P_2}$ such that a word $w$ is accepted to $A_{P_2}$ iff 
 the instance $I_w$ associated to $w$ enriched by the intentional predicates of $P_2$ and  by considering the values assigned to the $\lambda$ variables of $P_2$
as constants, $P_2$ satisfies $I_w$.



First, we can notice that if a connected conjunctive query $Q$ is mapped to $I_w$ then there a number $M_Q$ such that
for each mapping $\nu$ from $Q$ to $I$, the facts mapped by $\nu$  belong to a  sequence of consecutive nodes which is polynomial in $Q$.  

Secondly we assume that all the rules in $P_2$ are connected.
We present an algorithm that shows that given a word witness of $P_1$ , enriched by the intentional predicates and the $\lambda$ symbols of $P_2$,
checks that $P_2$ is satisfied by reading $I_w$ one way from the left to the right.
The idea is the following, when reading a node, the informations are kept to be sure to witness that each intentional predicate of $P_2$
in $I_w$ can be derived using the facts in the nodes. Without loss of generalities, there exists $M$ polynomial in $P_2$ such that 
it is sufficient to keep in memory  all the informations for witnessing all
the intentional predicates in the $M$ nodes on the right of the current nodes and the $M$ nodes on the left of the current node.
Let $q$ be the biggest query appearing in a body of $P_2$.
Because each rule of $P_2$ is connected, it is impossible to use the facts in the current node to witness an intentional predicate appearing in node
further  than $M_{q}$ nodes. Because in each node, there is a polynomial number of intentional predicates, we need to keep in memory after reading a node
the updates informations to witness an polynomial number of intentional predicates. A witness of the fact that a intentional predicate is derived 
is a CQ defining the body of a rule of size polynomial in $P_2$.  
When arriving in a node, the set of intentional predicates of the node reachable $M_q$ step is guessed and
for each of its intentional predicate $P$,  a mapping from a conjunctive
query defining the body of a rule of $P$ is guessed. After reading each node, the algorithm checks if guessed mapping is correct following the information of the node.
Finally, the cloture transitive of the dependences between the intentional facts appearing the nodes of the good window
 is updated and the algorithm ensures that there is not strongly connected
component of in the graph defined by the clotures transitive of dependences. An intentional fact $P$ is dependent of $P_1$ if $P_1$ is used in the witness mapping
of $P$. By assuring that the graph does not have any strongly connected component we ensure that the algorithm computes a proof tree of $P_2$.
The algorithm accepts a witness if each transition is correct and that the goal predicate appears in the witness.
We can notice that this algorithm uses only an polynomial memory at each step.
We can notice that this algorithm can simulated by an exponential non deterministic automaton $A_{P_2}$ over the alphabet $\Sigma_{P_1,P_2}$.
Let $A'_{P_2}$ be the automaton obtained from the projection of $A_{P_2}$ over $\Sigma_{P_2}$.
We can notice that a word $I$ is accepted by $A'_{P_2}$ iff its associated instance $I_{w}$ satisfies $A'_{P_2}$.
Therefore, $P_1$ is contained in $P_2$ iff $A_{P_1}$ is contained in $A'_{P_2}$
Because the containment of two non deterministic automata is in \PSpace and that $A_{P_1}$ and $A_{P_2}$ are in atmost exponential size then  
the containment of \linmdatalog in \mq is in \ExpSpace.  


==> noconstants.tex <==
\section{Monadic Datalog without Constants}\label{sec:noconstants}

\begin{theorem}
\containmentMembershipStatement{\mdatalog}{\gq}{\TwoExpTime}
\end{theorem}

\begin{theorem}
\containmentMembershipStatement{\mdatalog}{\kgq{k}}{\kExpTime{$(k+1)$}}
\end{theorem}

\begin{theorem}[\todo{know result by Vardi; add reference}]
\containmentHardnessStatement{\mdatalog}{\ucq}{\TwoExpTime}
\end{theorem}

\begin{theorem}
\containmentHardnessStatement{\mdatalog}{\kctworpq{k}}{\kExpTime{$(k+1)$}}
\end{theorem}

\begin{theorem}
\containmentMembershipStatement{\linmdatalog}{\mq}{\ExpSpace}
\end{theorem}
\begin{proof}
\input{linmdatalog-linMQ}
\end{proof}


\todo{The following is an optional remark (based on Vardi's construction for the non-nested case).}
\containmentMembershipStatement{\datalog}{\kgq{k}}{\kExpTime{$(k+1)$}}


==> related.tex <==
\subsection{Related Works}
\paragraph{Datalog}
Datalog is the classical language to define recursive queries over relational databases.
The static analyse of this language andsubfragment has been deeply studied for more than two decades and
in particular the problem of containment of two programs.

%The main question on static analyse for query languages is the question of the containment of a query $Q_1$ in another $Q_2$,
%i.e. if for each instance $I$, if $Q_1$ is satisfied by $I$ then $Q_2$ is satisfied by $I$.
% This question is useful for the optimization
%of queries.

 Unfortunately, the problem of containment of two datalog programs is undecidable\cite{Shm87}. 

There exists  two main restrictions that have studied making the contianment problem decidable: monadic datalog and nonrecursive datalog.

{\bf Monadic Datalog}
A monadic datalog program is a program containing only unary intentional predicates.

The problem of containment of monadic datalog program is \TwoExpTime complete. The upper-bound is well known and proven in \cite{Cosmadakis88}.
The hardness has been recently proven in \cite{BenediktBS12}. Finally, the containment of datalog program in a monadic datalog program is also decidable. 
It is a straightforward application\footnote{We thank Michael Benedikt to point us this result} of Theorem 5.5 of \cite{Courcelle91}.
However, the tight bounds for this last result are not known.  

{\bf Non-recursive datalog program and Union of conjunctive queries}
A non recursive datalog program does not have any recursion ans it is equivalent to an union of conjunctive queries. 
The problem of containment of a datalog program in an union of conjunctive queries is
$2$-{\sc exptime}-complete \cite{ChaudhuriV97}. Due to the succintness of non recursive datalog compare to union of conjunctive queries,
the  problem of containment of a datalog program in an union of
conjunctive queries is \ThreeExpTime-complete, \cite{ChaudhuriV97}.
Some restrictions for decreasing the complexity of these problems have been considered in \cite{ChaudhuriV94} and \cite{ChaudhuriV97}. 
A linear datalog program has rules with  bodies containing at most one intentional predicate.
 The problem of containment of a linear datalog program in a union of conjunctive queries is \ExpSpace-complete
and the complexity decreases to \PSpace when the linear datalog program is monadic.

Intuitively, the techniques to prove the upper bounds in the previous results 
are based on the reduction to the problem of containment of tree automaton for the general case and to the containment of automata when datalog programs are linear.

\pierre{The following is not necessary}
\begin{itemize}
\item If there exists a witness showing that a program $P_1$ is not contained in another program $P_2$ then there exists another witness which has a tree-like structure
which is obtained from the tree proof of $P_1$. 
\item The proof trees can be abstracted to trees and the set of these trees is regular and denoted $A_1$. The satisfaction of $P_2$ over a proof tree
can be reduced to the acceptation of the abstraction of the proof tree by a tree automaton $P_2$.
\end{itemize}

%Therefore, the previous problems of containment can be reduced to the containment of tree automaton for the general case and to the containment of automaton
%for the linear case. 

{\bf Extension of monadic datalog} 
Different propositions were made to extend the previous results for monadic programs: adding inequality predicate, extension to general intentional predicates,
queries based on monadic datalog programs.

{\bf Inequalities}
First, \cite{LevyMSS93} extends Monadic Datalog by allowing  inequalities predicates or negation of predicates in the body of the rules.
 Unfortunately, this extension leads to the undecidability of the containment problem for this language.
\pierre{This can be removed if necessary} It exhibits that the fact that witnesses
of the not containment of a program into another are closed under homomorphisms\footnote{i.e. that if $I$ is a witness of the not containment of $P_1$ in $P_2$
and that $I'$ satisfies $P_1$ and there exists an homomorphism from $I'$ to $I$ then $I'$ is a witness of the not containment of $P_1$ in $P_2$}
 is a key feature for the decidability of the containment of fragments of Datalog.

{\bf Guarded Datalog} 
A Guarded Datalog program  allows the use of intentional predicates with unrestricted arities, however for each rule, the variables of the head should
appear in a single extensional atom appearing in the body of the rule.
it has been introduced in \cite{BaranyCO12}.  They proved that the containment of Guarded Datalog is \TwoExpTime-complete. 
As notified in \cite{BaranyCO12}, a monadic datalog program can be rewritten in a guarded datalog program
as the only variable appearing in the head of a rule of a monadic datalog program can always be made guarded.  
Guarded Datalog can be extended to Guarded Negation Datalog by also allowing negated atoms guarded as explained previously. 
The containment of Guarded Negation Datalog programs remains \TwoExpTime-hard. 
These results are based on the decidability of the satisfiability
of the guarded negation fixed point logic introduced and studied in \cite{BaranyCS11}.

{\bf Nested monadically defined queries}
These languages have been introduced in \cite{RK13:flagcheck}. 
 Intuitively, a monadically defined query $Q$ is defined by
by a set of free variables $X$ and a monadic datalog program $P$ where these variables appears. 
$Q$ is satisfied over an instance $I$ iff there exists a valuation $\nu$  of the free variables in the values of $I$ such that the monadic datalog $P_{\nu}$
is satisfied by $I$. $P_{\nu}$
is obtained from 
$P$ by instantiating the free variables in the rules of $P$  by the mapped values. These values are then seen as constants of the program $P_{\nu}$.
The nested monadically defined query are defined as monadically defined queries and by  allowing 
the unrestricted use of relations defined by nested monadically programs.  
For both languages, the containment of programs is decidable \cite{RK13:flagcheck}.
The proof is the application of Theorem 5.5 of \cite{Courcelle91}.



%Datalog overview \cite{Alice}
%Emptiness decidable; Undecidability of containment of Datalog \cite{Shmueli93},

%Decidables cases: 
%Monadic Datalog : Upper bound \cite{Cosmadakis88}, Lower bound \cite{BenediktBS12} 
%Linear case \cite{ChaudhuriV94}


%Extensions with Negations/Inequalities/Functional Dependencies
%\cite{LevyMSS93}	

%Datalog in non recursive queries: 
%\cite{ChaudhuriV97}

\paragraph{Queries over graphs}
Graph are relationnal databases with relations of arity two.
A language of queries, conjunctive two way regular path queries, based on regular languages, has been deepely studied for one decade.
Intuively, a query in CR2PQ is a conjunct of atoms of the form $xLy$ where $L$ is a two way regular language. A pair of nodes $(n_1,n_2)$ 
is a valuation of the pair $(x,y)$ iff there exists a path between $n_1$ and $n_2$ accepted by $L$.
The containment of queries in this language is shown \ExpSpace-complete in \cite{regularpathqueries1,CalvaneseGLV03,AbiteboulV99,Deutsch2001}.
The containment of datalog program in a CR2PQ is in \TwoExpTime-complete \cite{CalvaneseGV05}.
Following \cite{RK13:flagcheck}, CR2PQ are expressible in monadically defined queries. 
Recently, a notion of nested Regular path queries has been introduced in \cite{BarceloLLW12}.
This language and CR2PQ are incomparables even though both are based on regular path. 
The containment of nested regular path queries  is in  \PSpace, \cite{Reutter13}.  

%Datalog in C2RPQs\cite{CalvaneseGV05}, 
%Containment of CR2PQs \cite{CalvaneseGLV03},
%Constraints \cite{AbiteboulV99},

%Nested Regular path queries:
%\cite{BarceloLLW12}

%Path Queries with Data 
%\cite{LibkinV12}

%Reasoning on Path 
%\cite{BarceloFL12}

%Guarded Datalog
%\cite{BaranyCO12}
%\cite{BaranyCS11}


%MODEQ
%\cite{RK13:flagcheck}






==> resume-copy.tex <==
\begin{tabular}{|l|c|c|c|c|c|}
\hline
     & \ucq,               &             & &  & \\
  & \linmdatalogconst{},  \mdatalogconst,  & \klinmq{k},  &  \kmq{k}, & \nmq, &  \\
  & \lingdatalog{},   \gdatalog  & \klingq{k}  &   \kgq{k} & \ngq & \datalog \\
\hline
\linmq
 &   \PSpace-h \cite{ChaudhuriV94} & \kExpSpace{$k$}-h  [Th.\ref{theo_hardlinmqklinmq}] &  \kExpSpace{$(k+1)$}-c & Nonelementary & Undecidable \cite{Alice} \\
&     \ExpSpace [Th.\ref{theo_memblindlgdl}]       &    \kExpSpace{$(k+1)$} [Th.\ref{theo_memblindlklingq}]   &   [Th.\ref{theo_memblindlgdl}]$\setminus$[Th.\ref{theo_memblindlklingq}] &  & \\
\hline
\lingdatalog,
 &  \ExpSpace-c & \kExpSpace{$(k+1)$}-c  & \kExpSpace{$(k+1)$}-c  & Nonelementary & Undecidable \cite{Alice}  \\
\klinmq{n} ($n \geq 2$),
 &  &  &  &  & \\
\klingq{n}, \lindatalog
 &     [Th.\ref{theo_hardtwolinmqklinmq}]$\setminus$[Th.\ref{theo_memblindlgdl}]       &       [Th.\ref{theo_hardlingqklinmq},\ref{theo_hardtwolinmqklinmq}]$\setminus$[Th.\ref{theo_memblindlklingq}] &
 [Th.\ref{theo_hardlingqklinmq},\ref{theo_hardtwolinmqklinmq}]$\setminus$[Th.\ref{theo_memblindlklingq}]  &   & \\
\hline
%\klinmq{n}, $n \geq 2$
% &  \ExpSpace-c & \kExpSpace{$(k+1)$}-c  &\kExpSpace{$(k+1)$}-c   & Undecidable  \\
%\hline
%\klingq{n}
% &  \ExpSpace-c & \kExpSpace{$(k+1)$}-c   & \kExpSpace{$(k+1)$}-c  & Undecidable  \\
%\hline
%\lindatalog
% &    \ExpSpace-c &  \kExpSpace{$k+1$}-c     & \kExpSpace{$(k+1)$}-c  & Undecidable \\
% &                            &                          &  Th.\ref{theo_memblindlklingq} & \\
\hline
\mdatalogconst, \gdatalog,
                   &  \TwoExpTime-c                                  & \kExpTime{$(k+2)$}-c &                    \kExpTime{$(k+2)$}-c  & Nonelementary & Undecidable \\
 \kmq{n}$\!\!$, \kgq{n}$\!\!$, & \cite{BenediktBS12,ChaudhuriV97}$\setminus$       &  [Th.\ref{theo_hardmdlmqk}]$\setminus$[Th.\ref{theo_membdlgqk}]          &     & & \\
% \nmq, \ngq, &    &  &     & & \\
 \nmq$\!\!$, \ngq$\!\!$, \datalog         & \cite{Cosmadakis88}, [Th.\ref{theo_membdlgdl}] &                                         &   [Th.\ref{theo_hardmdlmqk}]$\setminus$[Th.\ref{theo_membdlgqk}] & & \\
\hline
\end{tabular}

